Efficient Toxic Content Detection by Bootstrapping and Distilling Large Language Models

Toxic content detection is crucial for online services to remove inappropriate content that violates community standards. To automate the detection process, prior works have proposed varieties of machine learning (ML) approaches to train Language Models (LMs) for toxic content detection. However, both their accuracy and transferability across datasets are limited. Recently, Large Language Models (LLMs) have shown promise in toxic content detection due to their superior zero-shot and few-shot in-context learning ability as well as broad transferability on ML tasks. However, efficiently designing prompts for LLMs remains challenging. Moreover, the high run-time cost of LLMs may hinder their deployments in production. To address these challenges, in this work, we propose BD-LLM, a novel and efficient approach to Bootstrapping and Distilling LLMs for toxic content detection. Specifically, we design a novel prompting method named Decision-Tree-of-Thought (DToT) to bootstrap LLMs' detection performance and extract high-quality rationales. DToT can automatically select more fine-grained context to re-prompt LLMs when their responses lack confidence. Additionally, we use the rationales extracted via DToT to fine-tune student LMs. Our experimental results on various datasets demonstrate that DToT can improve the accuracy of LLMs by up to 4.6%. Furthermore, student LMs fine-tuned with rationales extracted via DToT outperform baselines on all datasets with up to 16.9\% accuracy improvement, while being more than 60x smaller than conventional LLMs. Finally, we observe that student LMs fine-tuned with rationales exhibit better cross-dataset transferability.

==> docs/rebuttal.tex <==
\noindent\textbf{Common Responses}\\
\noindent\textbf{1. Appropriateness for the track [Review 2, 4]:} 
According to the call for papers of this track, it covers topics related to safety, robustness, interpretability, and explainability of AI-based systems. We summarize the contributions of our paper for this track as follows: 
1) Our approach enhances the robustness of LLM-based toxic content detection systems, by iteratively selecting more fine-grained context and re-prompting LLMs to obtain more confident answers. 
2) Our approach improves the explainability of LLM-based toxic content detection systems, by making them generate high-quality rationales to better explain their answers. 
3) Experimental results on real-world datasets demonstrate that the proposed approach significantly improves over existing AI-based toxic content detection systems, which helps service providers to protect users from harmful content more effectively. We will revise Section 1 to make this clear.


\noindent\textbf{2. Motivation of DToT [Review 4, 5]:} 
Because there are many different types of toxic content and for each of them we need to use the right context (context refers to the part of the prompt that specifies the criteria to call certain content as toxic), there is a need to automatically select the appropriate context for each statement.
To solve this challenge, we design DToT prompting, which can automatically decide when to select more fine-grained context and which type of fine-grained context should be selected to boost LLMs' detection performance. Compared with baselines, DToT significantly boosts LLMs' detection performance by effectively selecting the most relevant fine-grained context. Moreover, DToT is more efficient since it only re-prompts LLMs when they generate low confidence answers. We will revise Section 3 to make this motivation more clear.

\noindent\textbf{3. Writing issues [Review 4, 5, 6]:} We will polish the paper to fix all formatting and writing errors, make the annotation and approach description in Section 3 more clear, and include more detailed explanation of zero-shot/few-shot in context learning. We will also release the source code link.

%Therefore, it is challenging to select the there are lots of detailed definitions about which content is toxic, such as the categories and subcategories of toxic content. In order for LLMs to make better decisions, it needs to know more fine-grained definitions about toxic content. Decision tree of thought can iteratively help to decide which type of fine-grained contexts are needed for LLMs, in order for it to make better decisions.  It can not only improve the detection accuracy of LLMs, but also reduce the context size in prompt by only providing the fine-grained context needed for LLMs’ decision. For example, if the LLM is confused about whether the sentence contains violent content or not, then it makes sense to provide context related to violent content only.

\vspace{.02in}
\noindent\textbf{Responses to Review 2}\\
\noindent\textbf{1. Challenges of prompt design:} Important challenges of prompt design for LLMs that we focus on include but are not limited to: 1) how to select demonstrations to boost the correctness of LLM responses; 2) how to select proper grounding information to enhance the trustworthiness of LLM responses; 3) how to design prompts to improve the consistency of LLM responses. We will revise the related text and add more references in Section 1.

\noindent\textbf{2. Evaluation of generated answers and rationales:} We clarify that the generated answers are either `yes' or `no'. Hence, it is sufficient to evaluate them using quantitative metrics such as accuracy (see Table 2 in Section 5). Additionally, we have qualitatively evaluated the generated rationales by comparing their length and richness in Section 5.2 (see subsection Q5). Moreover, we have provided examples of rationales generated by our approach and existing approaches in Appendix B (see Table 5) , which demonstrate that our approach significantly improves over existing approaches. We will update Section 5 to make this more clear.

\vspace{.03in}
\noindent\textbf{Responses to Review 3}\\
\noindent\textbf{1. Design novelty for white-box LLMs:} We clarify that the novelty for white-box LLMs is not the LLMs themselves, but the proposed DToT prompting for white-box LLMs. To the best of our knowledge, the proposed DToT for white-box LLMs is the first-of-its-kind design and implementation for enhancing the classification confidence of LLMs, which includes a novel context tree and context selector for effectively selecting more fine-grained context to prompt LLMs. Moreover, our paper is the first-of-its-kind study on bootstrapping and distilling LLMs for toxic content detection. We will revise the text to make this more clear.

\noindent\textbf{2. Performance of traditional deep learning methods:} We did compare our approach with the best performing traditional deep learning method, i.e. Bert-based models (see Section 5 comparison with RoBerta, which is a SOTA Bert-based model, and associated discussion in Section 4.2). Specifically, we show that our approach significantly outperforms RoBerta on all datasets with up to 16.9\% (see Table 2 in Section 5). We will revise the text to make this more clear.


\vspace{.02in}
\noindent\textbf{Responses to Review 4}\\
\noindent\textbf{1. Toxicity rating of black-box LLMs:} We explicitly ask black-box LLM to rate the toxicity level during prompting (see prompt templates in Table 6 of Appendix C in supplementary file). We will update the text to make it more clear.

\noindent\textbf{2. Threshold of confidence score:} We clarify that setting the threshold of confidence score as 0.9 improves the confidence of generated answers and thus enhances the overall detection accuracy. Note that during experiments, we empirically verified that answers with higher confidence lead to higher detection accuracy. Therefore, we select a confidence threshold of 0.9 to keep high-confident answers only. While for low confident answers, DToT will select more fine-grained context and re-prompt LLMs to boost their confidence. We will revise the text to make this more clear.

\vspace{.02in}
\noindent\textbf{Responses to Review 5}\\
\noindent\textbf{1. Performance of DToT+FS+R:} We clarify that the rationale used in DToT+FS+R for each demonstration is generated by LLMs (see Section 3.2), which may have low quality. When including low-quality rationales in DToT+FS+R, this may degrade LLMs' detection performance compared with DToT+FS. Specifically, as demonstrated in Table 2 of Section 5.1, LLMs achieve higher accuracy on Toxigen dataset but lower accuracy on SBIC and DHate datasets. This indicates that the rationales used in DToT+FS+R likely have higher quality on Toxigen dataset, but lower quality on SBIC and DHate datasets. Therefore, DToT+FS+R achieves the best performance on Toxigen dataset, but not on SBIC and DHate datasets. We will add text to make this more clear.

\vspace{.02in}
\noindent\textbf{Responses to Review 6}\\
\noindent\textbf{1. Demonstration of questions and responses:} We provided example responses in Table 5 of Appendix B and the prompt templates (i.e. questions asked) in the Table 6 of Appendix C. While we did point to the appendix from the main body, we will update the text to make this more clear.

\noindent\textbf{2. Input rationale of context selector:} As defined in Eq. (3) of Section 3.1, the input rationale of the context selector at step $t+1$ is the rationale generated by LLM at step $t$ (i.e. $r_t$). We will revise the text to make this more clear.

% \noindent\textbf{3. Explanations of zero-shot/few-shot in context learning:}
% In zero-shot in context learning, no example questions and answers will be provided as demonstration in the prompt. While in few-shot in context learning, a few example questions and answers will be provided as demonstration in the prompt. Our approach is orthogonal to few-shot learning, since it can be combined with existing methods on few-shot in-context learning to further improve the detection accuracy. We will clarify them and add more references in the camera-ready version.

% \noindent [1]\\
% \noindent [2]\\
% \noindent [3] Wang, X.; Wei, J.; Schuurmans, D.; Le, Q.; Chi, E.; Narang, S.; Chowdhery, A.; and Zhou, D. 2022b. Self-consistency improves chain of thought reasoning in language models. arXiv preprint arXiv:2203.11171.

